Wasserstein Contrastive Representation Distillation

The primary goal of knowledge distillation (KD) is to encapsulate the information of a model learned from a teacher network into a student network, with the latter being more compact than the former. Existing work, e.g., using Kullback-Leibler divergence for distillation, may fail to capture important structural knowledge in the teacher network and often lacks the ability for feature generalization, particularly in situations when teacher and student are built to address different classification tasks. We propose Wasserstein Contrastive Representation Distillation (WCoRD), which leverages both primal and dual forms of Wasserstein distance for KD. The dual form is used for global knowledge transfer, yielding a contrastive learning objective that maximizes the lower bound of mutual information between the teacher and the student networks. The primal form is used for local contrastive knowledge transfer within a mini-batch, effectively matching the distributions of features between the teacher and the student networks. Experiments demonstrate that the proposed WCoRD method outperforms state-of-the-art approaches on privileged information distillation, model compression and cross-modal transfer.

==> mv2BK.tex <==
\textbf{Ablation Study}
% \jj{Should this be merged with the ablation study at the end of 5.1?} 
We report results using only global or local contrastive knowledge transfer in Table \ref{tb:cifar100_same} and \ref{tb:cifar100_diff}. 
LCKT performs better than KD but slightly worse than CRD and GCKT, as both
CRD and GCKT are NCE-based algorithms, where negative samples are used to improve performance.
Additionally, GCKT enforces an 1-Lipschitz constraint on the critic function, which includes an extra hyper-parameter. 
% \jj{Is this the reason why WD performs slightly worse?}\lc{WD slightly worse is because it did not utilize negative samples}
Results show that CRD and GCKT have comparable results, and
in some cases, GCKT performs slightly better (\emph{e.g.}, from VGG13 to VGG8).

\input{table/ablation_parameter_modelcompression.tex}
We perform an additional ablation study on the weight of the $\Lcal_{\text{LCKT}}$ loss term (\emph{i.e.}, $\lambda_2$ in (\ref{eq:wcord})). We adjust $\lambda_2$ from $0$ to $0.2$, and set $\lambda_1=0.8$, which is the same as in CRD for fair comparison.
  Results are summarized in Table \ref{tb:cifar100_ablation}. The standard deviation (Std) is reported based on 5 runs.
We observe that:
($i$) when $\lambda_2=0.05$, ResNet-8x4 performs the best; and ($ii$) WCoRD can consistently outperform GCKT and CRD methods, when $\lambda_2\in(0,0.2]$. 
% \vspace{-2mm}

\textbf{Experiments on ImageNet}
We also evaluate the proposed method on a larger dataset,
ImageNet~\citep{deng2009imagenet}, which contains $1.2$M images for training and $50$K for validation.
In this experiment, we use ResNet-34~\cite{he2016deep} as the teacher and ResNet-18 as the student, and use the same training setup as in CRD~\cite{tian2019contrastive} for fair comparison.
Top-$1$ and Top-$5$ error rates (lower is better) are reported in Table ~\ref{tb:imagenet}, showing that the 
%
WCoRD+KD method achieves the best student performance on the ImageNet dataset.
The relative improvement of WCoRD over CRD on Top-1 error is $44.4\%$, and the relative improvement on Top-5 error is $23.08\%$.
Such significant improvement on a large dataset like ImageNet demonstrates the scalability of our method.


\textbf{Ablation Study} We investigate the importance of the local knowledge transfer term  $\Lcal_{\text{LCKT}}(\cdot)$ in WCoRD. As shown in Tables \ref{tb:cifar100_same} and \ref{tb:cifar100_diff}, without it, WCoRD cannot consistently outperform CRD in different student-teacher architecture settings. 
By fixing $\lambda_1$ for the $\Lcal_{\text{GCKT}}(\cdot)$ loss with $\lambda_1=1$, we adjust the hyper-parameter $\lambda_2$ from $0.01$ to $0.2$. Table \ref{tb:privilege_ablation} reports the results, where it is evident that %accuracy of the last-training-epoch model and the best model.
with $\lambda_2=0.07$ WCoRD performs the best. 
Also, we observe that when choosing $\lambda_2$ from $(0,0.1]$, it is consistently better than the model variant with $\lambda_2=0$. This indicates that our model is relatively robust given different hyper-parameter choices.

==> table/relativeImprove_1.tex <==

\begin{table*}[ht]

\setlength{\tabcolsep}{4.5pt}
\begin{center}
\begin{tabular}{lccccccc}
\toprule
\thead{ \\ } & \thead{WRN-40-2 \\ WRN-16-2} & \thead{WRN-40-2 \\ WRN-40-1} & \thead{resnet56\\resnet20} & \thead{resnet110\\resnet20} & \thead{resnet110\\resnet32} & \thead{resnet32x4\\resnet8x4} & \thead{vgg13\\vgg8}\\
\midrule
CRD-KD    & 2.22 & 0.60 & 0.50 & 0.79 & 0.40 & 2.18 & 0.96 \\
WCoRD-CRD & 0.40 & 0.59 & 0.40 & 0.11 & 0.33 & 0.44 & 0.61 \\
Relative Improvement (\%) & 18.0 & 98.3 & 80 & 13.9 & 82.5 & 20.2 & 63.5 \\ 
\midrule
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{
\small{relative improvement
}}
\label{tb:cifar100_same}
\end{center}
% \vspace{-10pt}
\end{table*}
